Multipath-based SLAM for Non-Ideal Reflective Surfaces Exploiting Multiple-Measurement Data Association

Multipath-based simultaneous localization and mapping (SLAM) is a promising approach to obtain position information of transmitters and receivers as well as information regarding the propagation environments in future mobile communication systems. Usually, specular reflections of the radio signals occurring at flat surfaces are modeled by virtual anchors (VAs) that are mirror images of the physical anchors (PAs). In existing methods for multipath-based SLAM, each VA is assumed to generate only a single measurement. However, due to imperfections of the measurement equipment such as non-calibrated antennas or model mismatch due to roughness of the reflective surfaces, there are potentially multiple multipath components (MPCs) that are associated to one single VA. In this paper, we introduce a Bayesian particle-based sum-product algorithm (SPA) for multipath-based SLAM that can cope with multiple-measurements being associated to a single VA. Furthermore, we introduce a novel statistical measurement model that is strongly related to the radio signal. It introduces additional dispersion parameters into the likelihood function to capture additional MPCs-related measurements. We demonstrate that the proposed SLAM method can robustly fuse multiple measurements per VA based on numerical simulations.

==> inputFiles/Wgroup-Teaching-Preamble.tex <==
% Greek lowercase letters, sans serif font - by Guido

%\@ifpackageloaded{<name>}{<true>}{<false>}
\usepackage{bm}

%% =========== Euler ==========
%\DeclareMathAlphabet{\matheur}{U}{eur}{m}{n}
%\SetMathAlphabet{\matheur}{bold}{U}{eur}{b}{n}
%\DeclareRobustCommand{\msf}[1]{%
%  \ifcat\noexpand#1\relax\msfgreek{#1}\else\matheur{#1}\fi%for math sans serif (Euler)
%}
%% =========================
%
%% ==== Computer Modern Sans Serif ====
\DeclareMathAlphabet{\mathsfbr}{OT1}{cmss}{m}{n}%for math sans serif (cmss)
\SetMathAlphabet{\mathsfbr}{bold}{OT1}{cmss}{bx}{n}%for math sans serif (cmss)
\DeclareRobustCommand{\msf}[1]{%
  \ifcat\noexpand#1\relax\msfgreek{#1}\else\mathsfbr{#1}\fi%for math sans serif (cmss)
}
%% =========================

% ==== Computer Modern Bright ====
%% Part 1: This is necessary to fix a bug in the .fd file of the font!!!
%\DeclareFontFamily{OT1}{cmbr}{\hyphenchar\font45 }
%\DeclareFontShape{OT1}{cmbr}{m}{n}{%
%  <-9>cmbr8
%  <9-10>cmbr9
%  <10-17>cmbr10
%  <17->cmbr17
%}{}
%\DeclareFontShape{OT1}{cmbr}{m}{sl}{%
%  <-9>cmbrsl8
%  <9-10>cmbrsl9
%  <10-17>cmbrsl10
%  <17->cmbrsl17
%}{}
%\DeclareFontShape{OT1}{cmbr}{m}{it}{%
%  <->ssub*cmbr/m/sl
%}{}
%\DeclareFontShape{OT1}{cmbr}{b}{n}{%
%  <->ssub*cmbr/bx/n
%}{}
%\DeclareFontShape{OT1}{cmbr}{bx}{n}{%
%  <->cmbrbx10
%}{}
%% Part 2
%\DeclareMathAlphabet{\mathsfbr}{OT1}{cmbr}{m}{n}%for math sans serif bright (cmbr)
%\SetMathAlphabet{\mathsfbr}{bold}{OT1}{cmbr}{b}{n}%for math sans serif bright (cmbr)
%\DeclareRobustCommand{\msf}[1]{%
%  \ifcat\noexpand#1\relax\msfgreek{#1}\else\mathsfbr{#1}\fi%for math sans serif bright (cmbr)
%}
%% =========================

\makeatletter
\newcommand{\msfgreek}[1]{\csname s\expandafter\@gobble\string#1\endcsname}
\makeatother

% Sans serif greek
\DeclareFontEncoding{LGR}{}{} % or load \usepackage{textgreek}
\DeclareSymbolFont{sfgreek}{LGR}{cmss}{m}{n}
\SetSymbolFont{sfgreek}{bold}{LGR}{cmss}{bx}{n}
\DeclareMathSymbol{\salpha}{\mathord}{sfgreek}{`a}
\DeclareMathSymbol{\sbeta}{\mathord}{sfgreek}{`b}
\DeclareMathSymbol{\sgamma}{\mathord}{sfgreek}{`g}
\DeclareMathSymbol{\sdelta}{\mathord}{sfgreek}{`d}
\DeclareMathSymbol{\sepsilon}{\mathord}{sfgreek}{`e}
\DeclareMathSymbol{\szeta}{\mathord}{sfgreek}{`z}
\DeclareMathSymbol{\seta}{\mathord}{sfgreek}{`h}
\DeclareMathSymbol{\stheta}{\mathord}{sfgreek}{`j}
\DeclareMathSymbol{\siota}{\mathord}{sfgreek}{`i}
\DeclareMathSymbol{\skappa}{\mathord}{sfgreek}{`k}
\DeclareMathSymbol{\slambda}{\mathord}{sfgreek}{`l}
\DeclareMathSymbol{\smu}{\mathord}{sfgreek}{`m}
\DeclareMathSymbol{\snu}{\mathord}{sfgreek}{`n}
\DeclareMathSymbol{\sxi}{\mathord}{sfgreek}{`x}
\DeclareMathSymbol{\somicron}{\mathord}{sfgreek}{`o}
\DeclareMathSymbol{\spi}{\mathord}{sfgreek}{`p}
\DeclareMathSymbol{\srho}{\mathord}{sfgreek}{`r}
\DeclareMathSymbol{\ssigma}{\mathord}{sfgreek}{`s}
\DeclareMathSymbol{\stau}{\mathord}{sfgreek}{`t}
\DeclareMathSymbol{\supsilon}{\mathord}{sfgreek}{`u}
\DeclareMathSymbol{\sphi}{\mathord}{sfgreek}{`f}
\DeclareMathSymbol{\schi}{\mathord}{sfgreek}{`q}
\DeclareMathSymbol{\spsi}{\mathord}{sfgreek}{`y}
\DeclareMathSymbol{\somega}{\mathord}{sfgreek}{`w}
\let\svarepsilon\sepsilon
\let\svartheta\stheta
\let\svarpi\spi
\let\svarrho\srho
\DeclareMathSymbol{\svarsigma}{\mathord}{sfgreek}{`c}
\let\svarphi\sphi
\DeclareMathSymbol{\sGamma}{\mathalpha}{sfgreek}{`G}
\DeclareMathSymbol{\sDelta}{\mathalpha}{sfgreek}{`D}
\DeclareMathSymbol{\sTheta}{\mathalpha}{sfgreek}{`J}
\DeclareMathSymbol{\sLambda}{\mathalpha}{sfgreek}{`L}
\DeclareMathSymbol{\sXi}{\mathalpha}{sfgreek}{`X}
\DeclareMathSymbol{\sPi}{\mathalpha}{sfgreek}{`P}
\DeclareMathSymbol{\sSigma}{\mathalpha}{sfgreek}{`S}
\DeclareMathSymbol{\sUpsilon}{\mathalpha}{sfgreek}{`U}
\DeclareMathSymbol{\sPhi}{\mathalpha}{sfgreek}{`F}
\DeclareMathSymbol{\sPsi}{\mathalpha}{sfgreek}{`Y}
\DeclareMathSymbol{\sOmega}{\mathalpha}{sfgreek}{`W}

\DeclareRobustCommand{\mcal}[1]{%
  \ifcat\noexpand#1\relax\mathnormal{#1}\else\cal{#1}\fi
}
\DeclareRobustCommand{\BM}[1]{%
  \ifcat\noexpand#1\relax\bm{\boldUppercaseItalicGreek{#1}}\else\bm{#1}\fi
}
\makeatletter
\newcommand{\boldUppercaseItalicGreek}[1]{\csname var\expandafter\@gobble\string#1\endcsname}
\makeatother
%-------------------------
% Math symbol
%-------------------------
%\newcommand{\rv}[1]{\MakeLowercase{\msf{#1}}}  
%\newcommand{\RV}[1]{\bm{\MakeLowercase{\msf{#1}}}}
%\newcommand{\RM}[1]{\bm{\MakeUppercase{\msf{#1}}}}
%\newcommand{\RS}[1]{\MakeUppercase{\msf{#1}}}
\newcommand{\rv}[1]{\msf{#1}}
\newcommand{\RV}[1]{\bm{\msf{#1}}}
\newcommand{\RM}[1]{\bm{\msf{#1}}}
\newcommand{\RS}[1]{\msf{#1}}

\newcommand{\V}[1]{\bm{#1}}
\newcommand{\M}[1]{\BM{#1}}
\newcommand{\Set}[1]{{\mcal{#1}}}


==> inputFiles/acronyms_unsorted.tex <==
% Acronym definitions: SORT ALPHABETICALLY!!!! life's too short: in bash 'sort acronyms.tex > acronyms_sorted.tex'

\acrodef{pa}[PA]{physical anchor}
\acrodef{mimo}[MIMO]{multiple input multiple output}
\acrodef{awgn}[AWGN]{additive white Gaussian noise}
\acrodef{bw}[BW]{bandwidth}
\acrodef{blt}[BLT]{bluetooth}
\acrodef{cdf}[CDF]{cumulative distribution function}
\acrodef{crlb}[CRLB]{Cram\'er-Rao lower bound}
\acrodef{dmc}[DMC]{dense multipath component}
\acrodef{dut}[DUT]{device under test}
\acrodef{eirp}[EIRP]{equivalent isotropic radiated power}
\acrodefplural{esl}[ESLs]{electronic shelf labels}
\acrodef{los}[LOS]{line-of-sight}
\acrodef{mf}[MF]{matched filter}
\acrodef{ml}[ML]{maximum likelihood}
\acrodef{mpc}[MPC]{multipath component}
\acrodef{nlos}[NLOS]{non-\ac{los}}
\acrodef{pcb}[PCB]{printed circuit board}
\acrodef{pdf}[PDF]{probability density function}
\acrodef{reb}[REB]{ranging error bound}
\acrodef{rss}[RSS]{received signal strength}
\acrodef{smc}[SMC]{specular multipath component}
\acrodef{snr}[SNR]{signal-to-noise-ratio}
\acrodef{sinr}[SINR]{signal-to-interference-plus-noise-ratio}
\acrodef{tdoa}[TDOA]{time difference of arrival}
\acrodef{tka}[TKA]{trusted keyless access}
\acrodef{toa}[TOA]{time-of-arrival}
\acrodef{aoa}[AOA]{angle-of-arrival}
\acrodef{uwb}[UWB]{ultra wide band}
\acrodef{mie}[MIE]{method of interval estimation}
\acrodef{mc}[MC]{Monte Carlo}
\acrodef{mse}[MSE]{mean squared error}
\acrodef{ci}[CI]{confidence interval}
\acrodef{cl}[CL]{confidence level}
\acrodef{pdp}[PDP]{power delay profile}
\acrodef{dps}[DPS]{delay power spectrum}
\acrodef{dm}[DM]{dense multipath}
\acrodef{nlike}[NLIKE]{normalized likelihood}
\acrodef{zzb}[ZZB]{Ziv-Zakai bound}
\acrodef{ut}[UT]{unscented transform}
\acrodef{glrt}[GLRT]{generalized likelihood ratio test}
\acrodef{mse}[MSE]{mean squared error}
\acrodef{rmse}[RMSE]{root mean squared error}
\acrodef{nnlike}[NNLIKE]{normalized noise-free likelihood}
\acrodef{stdv}[STDV]{standard deviation}
\acrodef{rv}[RV]{random variable}
\acrodef{bp}[BP]{belief propagation}
\acrodef{pda}[PDA]{probabilistic data association}
\acrodef{mp}[MP]{multipath}
\acrodef{pmf}[PMF]{probability mass function}
\acrodef{pdaf}[PDAF]{probabilistic data association filter}
\acrodef{pdaai}[AIPDA]{amplitude-information \ac{pda}}
\acrodef{olos}[OLOS]{obstructed \ac{los}}
\acrodef{spa}[SPA]{sum-product algorithm}
\acrodef{mmse}[MMSE]{minimum mean-square error}
\acrodef{lhf}[LHF]{likelihood function}
\acrodef{fa}[FA]{false alarm}
\acrodef{ceda}[CEDA]{channel estimation and detection algorithm}
\acrodef{pcrlb}[PCRLB]{posterior Cram\'er-Rao lower bound}
\acrodef{slam}[SLAM]{simultaneous localization and mapping}
% \acrodef{mpslam}[MP-SLAM]{multipath-based SLAM}
\acrodef{va}[VA]{virtual anchor}
\acrodef{dnr}[DNR]{dense-to-noise ratio}
\acrodef{pbo}[PBO]{potential bias object}
\acrodef{npbo}[NPBO]{new \ac{pbo}}
\acrodef{lpbo}[LPBO]{legacy \ac{pbo}}

